Inferential Privacy Guarantees for Differentially Private Mechanisms

The correlations and network structure amongst individuals in datasets today---whether explicitly articulated, or deduced from biological or behavioral connections---pose new issues around privacy guarantees, because of inferences that can be made about one individual from another's data. This motivates quantifying privacy in networked contexts in terms of "inferential privacy"---which measures the change in beliefs about an individual's data from the result of a computation---as originally proposed by Dalenius in the 1970's. Inferential privacy is implied by differential privacy when data are independent, but can be much worse when data are correlated; indeed, simple examples, as well as a general impossibility theorem of Dwork and Naor, preclude the possibility of achieving non-trivial inferential privacy when the adversary can have arbitrary auxiliary information. In this paper, we ask how differential privacy guarantees translate to guarantees on inferential privacy in networked contexts: specifically, under what limitations on the adversary's information about correlations, modeled as a prior distribution over datasets, can we deduce an inferential guarantee from a differential one? We prove two main results. The first result pertains to distributions that satisfy a natural positive-affiliation condition, and gives an upper bound on the inferential privacy guarantee for any differentially private mechanism. This upper bound is matched by a simple mechanism that adds Laplace noise to the sum of the data. The second result pertains to distributions that have weak correlations, defined in terms of a suitable "influence matrix". The result provides an upper bound for inferential privacy in terms of the differential privacy parameter and the spectral norm of this matrix.

==> prelims.tex <==
%\subsection{Computing the networked privacy guarantee}
%\label{sec:prelims}
\label{s-prelim}
\noindent
We conclude this section with a brief discussion about
computing the networked privacy parameter of a
mechanism. Let $\ndp_{01}$ be defined as
in~\eqref{eq:def-ndp.2} but fixing $\val_0=0, \, \val_1=1$
in the maximization; similarly define $\ndp_{10}$ by fixing
$\val_0=1, \, \val_1=0$. Recalling the conditional
distributions $\cdl, \cdu$ defined earlier, we can
restate~\eqref{eq:def-ndp.2} in the form of a mathematical
program to compute the maximum of $e^{\ndp_{01}}$ over all
$\bm{\idp}$-differentially private mechanisms $\M$.
For ease of notation we assume $a=1$.
\begin{lemma} \label{lem:mp-ndp}
%% For a mechanism $\M$ let $\ndp_{01}$ be defined by
%% \BEQ \label{eq:lmp.1}
%% e^{\ndp_{01}} =  \max
%%                  \left\{  \left. \frac{\Pr(\M(\fdb)=\outc \given \ba=1)}
%%                                              {\Pr(\M(\fdb)=\outc \given \ba=0)}
%%                              \, \right| \, \outc \in \outcomes
%%                  \right\}.
%% \EEQ
%% Then 
For a given vector of differential privacy parameters, $\bm{\idp} = (\idp_1
,\ldots,\idp_n)$,
the maximum of $e^{\ndp_{01}}$ over all $\bm{\idp}$-differentially private mechanisms 
is equal to the optimum value of the non-linear program
\BEQ \label{eq:mp-ndp}
\begin{array}{rl}
\mbox{maximize}_{\m(\fdb)} & \frac{\sum_{\pdb \in \{0,1\}^{n-1}} \cdu({\pdb}) \m(1,\pdb)}{\sum_{\pdb \in \{0,1\}^{n-1}}  \cdl({\pdb}) \m(0, \pdb)} \\ 
\mbox{s.t.} & e^{-\idpi} \leq  \frac{\m({\fdb})} {\m({\adb})} \leq e^{\idpi} ~~\forall i, \fdb, \adb \mbox{ with } \fdb \sim_i \adb \\
&0 \leq \m({\fdb}) 
\end{array}
\EEQ
as well as the optimum of the linear program
\BEQ \label{eq:lp-ndp}
\begin{array}{rl}
\mbox{maximize}_{\m(\fdb)} & \sum_{\pdb \in \{0,1\}^{n-1}} \cdu({\pdb}) \m(1,\pdb) \\ 
\mbox{s.t.} & e^{-\idpi} \leq  \frac{\m({\fdb})} {\m({\adb})} \leq e^{\idpi} ~~\forall i, \fdb, \adb \mbox{ with } \fdb \sim_i \adb \\
&{\sum_{\pdb \in \{0,1\}^{n-1}}  \cdl({\pdb}) \m(0, \pdb)} = 1 \\
&0 \leq \m({\fdb}) 
\end{array}
\EEQ
\end{lemma}
\begin{proof}
For any mechanism $\M$, if we let $\outc$ denote the outcome that maximizes 
$\frac{\Pr(\M(\fdb)=\outc \mid \ba = 1)}{\Pr(\M(\fdb) = \outc \mid \ba=0)}$ and
set $\m(\fdb) = \m_\outc(\fdb)$ for every $\fdb$, then we obtain a feasible
solution of~\eqref{eq:mp-ndp}. Conversely, given any feasible solution we 
can rescale the values $\m(\fdb)$ by a common factor if necessary---the
objective function and the feasible region of~\eqref{eq:mp-ndp} are
invariant under scaling---and construct a mechanism $\M$ with two outcomes 
$\outc, \outc'$  by setting $\m_{\outc}(\fdb) = 1 - \m_{\outc'}(\fdb) = \m(\fdb)$
for every $\fdb$. The constraints of~\eqref{eq:mp-ndp} ensure that the
$\M$ satisfies $\bm{\idp}$-differential privacy with respect to outputting $\outc$.
To ensure that it also satisfies $\bm{\idp}$-differential privacy with respect 
to outputting $\outc'$ we can scale $\m(\cdot)$ down until the probabilities
$\m_{\outc'}(\fdb)$ are so close to 1 that they satisfy differential privacy automatically.
Finally, we can exploit the scale-invariance once more to justify that~\eqref{eq:mp-ndp}
and~\eqref{eq:lp-ndp} have the same optimum value.
\end{proof}


%% \BEQ \label{eq:mp-ndp} 
%% \begin{array}{rl}
%% \mbox{maximize}_{\m(\fdb)} & \frac{\sum_{\pdb \in \{0,1\}^{n-1}} \cdu({\pdb}) \m(1,\pdb)}{\sum_{\pdb \in \{0,1\}^{n-1}}  \cdl({\pdb}) \m(0, \pdb)} \\ 
%% \mbox{s.t.} & e^{-\idpi} \leq  \frac{\m({\fdb})} {\m({\adb})} \leq e^{\idpi} ~~\forall i, \fdb, \adb \mbox{ with } \fdb \sim_i \adb \\
%% &0 \leq \m({\fdb}) 
%% \end{array}
%% \EEQ
%% %% \ifextabs
%% %% We defer to Appendix~\ref{app:prelims} the (easy) proof that~\eqref{eq:mp-ndp}
%% %% correctly computes $e^{\ndp_{01}}$ and that it can be reformulated as a linear
%% %% program.
%% %% \else
%% \autoref{lem:mp-ndp} in the appendix formalizes the notion
%% that~\eqref{eq:mp-ndp} correectly computes the networked privacy
%% guarantee and that it is equivalent to a linear program. Here
%% we provide a brief sketch of the argument.
%% For any mechanism $\M$, if we let $\outc$ denote the outcome that maximizes 
%% $\frac{\Pr(\M(\fdb)=\outc \mid \ba = 1)}{\Pr(\M(\fdb) = \outc \mid \ba=0)}$ and
%% set $\m(\fdb) = \m_\outc(\fdb)$ for every $\fdb$, then we obtain a feasible
%% solution of~\eqref{eq:mp-ndp}. Conversely, given any feasible solution we 
%% can rescale the values $\m(\fdb)$ by a common factor if necessary---the
%% objective function and the feasible region of~\eqref{eq:mp-ndp} are
%% invariant under scaling---and construct a mechanism $\M$ with two outcomes 
%% $\outc, \outc'$  by setting $\m_{\outc}(\fdb) = 1 - \m_{\outc'}(\fdb) = \m(\fdb)$
%% for every $\fdb$. The constraints of~\eqref{eq:mp-ndp} ensure that the
%% $\M$ satisfies $\bm{\idp}$-differential privacy with respect to outputting $\outc$.
%% To ensure that it also satisfies $\bm{\idp}$-differential privacy with respect 
%% to outputting $\outc'$ we can scale $\m(\cdot)$ down until the probabilities
%% $\m_{\outc'}(\fdb)$ are so close to 1 that they satisfy differential privacy automatically.
%% Finally, note that although~\eqref{eq:mp-ndp} isn't written in the form of a linear
%% program, we can exploit the scale-invariance once more by adding an extra
%% constraint $\sum_{\pdb \in \{0,1\}^{n-1}}  \cdl({\pdb}) \m(0, \pdb)=1$,
%% which makes the objective function linear without changing the value of the optimum.
%% % \fi


%% RDK: Commenting out the following, which will need to be fleshed out and
%%          shortened.
\iffalse
\BIT 
\item Formulate the problem of computing NDP as a mathematical program. 
\tg{We first note that this problem of computing the networked differential privacy guaranteed by a given vector of individual differential privacy guarantees can be written as a mathematical program:
\BEQS
\begin{array}{rl}
\mbox{maximize}_{\m_{\fdb}} & \frac{\sum_{\db \in \{0,1\}^n} \cdu_{\db}\m(1 \db)}{\sum_{\db \in \{0,1\}^n}  \cdl_{\db}\m(0 \db)} \\ 
\mbox{s.t.} &\frac{1}{\alpha_i} \leq  \frac{\m_{\fdb}} {\m_{\fdb'}} \leq \alpha_i ~~\forall i, \fdb, \fdb' \mbox{ with } \fdb_i \neq \fdb'_{i}, \fdb_{-i} = \fdb'_{-i}\\
&0 \leq \m_{\fdb} \leq 1. 
\end{array}
\EEQS
(Recall that $\ai= \idpgi$ .)
The objective is the ratio in (\ref{e-ndpdef}) \tr{for a given outcome} for a mechanism $\M = \m_{\fdb}$ (for the given joint distribution $\cdu$, and the last constraint simply says that the $\m_{\db}$ are probabilities, and therefore must lie between zero and one. The first constraint encodes the individual differential privacy constraints that the mechanism $\M$ must satisfy: for each individual $i$, the ratio of the probabilities of returning the outcome $o$, $\frac{\m_{\fdb}} {\m_{\fdb'}}$, must be bounded by $\ai$ and $1/\ai$ respectively. (Note that there is no sum constraint on the probabilities since $\m_{\fdb}$ is the probability that $\M$ returns a {\em particular} outcome $o$ with input $\fdb$, \ie, $\m$ ranges over all databases and a single outcome, rather than all outcomes for a single database. 
}
\item \ttd{Discuss minimum issue: NDP is actually max of ratio and 1/min(ratio).} 
\item Get factor of $\aat$ out. 


First note that the program above is equivalent to a reduced problem with variables $\m_{\db}$, obtained by setting $\frac{\m_{1\db}} {\m_{0\db}} = \alpha_0$ for all $\db$:
\BEQ
\begin{array}{rl}
\label{e-ndpmp}
\mbox{maximize}_{\m_{\db}} & \aat \frac{\sum_{\db \in \{0,1\}^n} \cdu_{\db}\m(\db)}{\sum_{\db \in \{0,1\}^n}  \cdl_{\db}\m(\db)} \\ 
\mbox{s.t.} &\frac{1}{\alpha_i} \leq  \frac{\m_{\db}} {\m_{\db'}} \leq \alpha_i ~~\forall i = 1, \ldots, n, \fdb, \fdb' \mbox{ with } \fdb_i \neq \fdb'_{i}, \fdb_{-i} = \fdb'_{-i}\\
&0 \leq \m_{\fdb} \leq 1, 
\end{array}
\EEQ
since the ratio in the objective in the two programs are equal when $\frac{\m_{\fdb}}{\m_{\fdb'}} = \aat$ for all databases $\fdb, \fdb'$ that differ only in Athena's bit, and the ratio in the first program is maximized by maximizing the ratio $\frac{\m_{\fdb}}{\m_{\fdb'}}$ subject to IDP constraints. We will henceforth focus on this program as our NDP computation, and note that we can, without loss of generality, \tr{set $\m_{\db} = 1$ for $\db = 0\ldots 0$}, \ie, the all-zeros string. 

\item Independence and perfect correlation. 

First suppose that all individuals' bits are perfectly correlated, \ie, the probabilities of all bit strings $\fdb$ except the all-ones and all-zeros strings is zero. Then, $\cdu_{\db}= 1$ for $\db = \ones$ and $ \cdl_{\db} = 1$ for $\db = \zeros$, since $\cdu_{\db}$ and $\cdl_{\db}$ are the {\em conditional} probabilities of the remaining $n$ individuals' data being $\db$ given Athena's bit is $1$ (respectively $0$). The objective in (\ref{e-ndpmp}) is maximized by setting $\m$ so that $\frac{\m_{\fdb}}{\m_{\fdb'}} = \alpha_i$ for all relevant database pairs, \ie, so that the IDP constraint in (\ref{e-ndpmp}) is tight. 

Next consider the other extreme of independence: suppose Athena's bit and all other individuals' bits are independent. Then, $\cdu_{\db}= \cdl_{\db} = \jd_{\db}$ for all databases $\db$, where we abuse notation to let $\jd_{\db}$ denote the (unconditional) probability of the remaining $n$ individuals' bits taking on value $\db$. But this makes the numerator and the denominator in the ratio in the objective of (\ref{e-ndpmp}) equal, so that the objective value is exactly $\aat$ for all possible values of $\m_{\db}$---that is, {\em every} IDP mechanism provides the same NDP guarantee, equal to the IDP guarantee, to Athena, if her bit is independent of the remaining individuals' bits (irrespective of any correlations that might exist between those individuals' bits). And indeed, this is exactly as it should be, since independence is the ``least'' knowledge an adversary can have about correlations amongst individuals' data, in which case we should expect the network differential privacy guarantee to be exactly the same as the individual differential privacy guarantee, since there is---effectively---no network. 

In fact, these observations can be strengthened to show that the NDP guarantee always lies between the values at these two extremes of independence and perfect correlation, as summarized in the following theorem: 
\begin{theorem} 
\label{t-ndpbasic}
The NDP guarantee relates to the IDP guarantee as follows: 
\[ 
\idpa \leq \ndp \leq \idpa + \sum_{i=1}^n \idp_i. 
\] 
Further, (i) $\ndp = \idpa$ if and only if $\ba$ is independent of $\db$ and (ii) $\ndp = \idpa + \sum_{i=1}^n \idp_i$ if and only if all individuals' bits are perfectly correlated. 
\end{theorem} 
\tg{ (Proof in appendix: Analyze the dual of the LP to prove that IDP=NDP only when distribution is independent, and NDP = n*IDP only when the distribution is perfectly correlated.) }



\EIT 
\fi

